On the sojourn time of a batch in the $M^{[X]}/M/1$ Processor Sharing Queue

In this paper, we analyze the sojourn of an entire batch in a processor sharing $M^{[X]}/M/1$ processor queue, where geometrically distributed batches arrive according to a Poisson process and jobs require exponential service times. By conditioning on the number of jobs in the systems and the number of jobs in a tagged batch, we establish recurrence relations between conditional sojourn times, which subsequently allow us to derive a partial differential equation for an associated bivariate generating function. This equation involves an unknown generating function, whose coefficients can be computed by solving an infinite lower triangular linear system. Once this unknown function is determined, we compute the Laplace transform and the mean value of the sojourn time of a batch in the system.

==> data_matlab.tex <==
row= q x10;
col=rho* x 10
N=1M

meanW =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    2.8491    3.3163    4.0126         0         0    9.9698         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    7.1579    8.2916   10.0019         0         0   25.0974         0
         0         0   14.1056   16.5664   20.5566         0         0   50.7872         0

>> meanWb

meanWb =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    3.0543    3.6623    4.5951         0         0   13.3088         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    8.1252    9.9280   12.7173         0         0   42.1318         0
         0         0   16.3858   20.4420   27.2760         0         0   93.0302         
         
N=10M
meanWb =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    3.0678    3.6825    4.5745         0         0   13.3884         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    8.1453    9.9327   12.7583         0         0   41.7556         0
         0         0   16.6219   20.5796   26.5404         0         0   91.6515         0


meanW =

         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    2.8592    3.3325    4.0011         0         0   10.0135         0
         0         0         0         0         0         0         0         0         0
         0         0         0         0         0         0         0         0         0
         0         0    7.1737    8.3009   10.0274         0         0   24.8916         0
         0         0   14.3206   16.6684   20.0237         0         0   50.0389         0


mean job &	mean batch& $q$	&$\rho^*$\\ \hline
2.8491 &	3.0543&	0.3&	0.5 \\
3.3163 &3.6623	& 	0.4& 	0.5 \\
4.0126 & 4.5951	 &	0.5	& 0.5 \\
9.9698 &	 13.3088	 & 0.8 &	0.5\\
\hline
7.1579 &	8.1252 &	0.3 &	0.8 \\
8.2916 &	9.9280 & 	0.4& 	0.8 \\
10.0019 &	12.7173 &	0.5	& 0.8 \\
25.0974 &	42.1318	 & 0.8 &	0.8 \\
\hline
 14.1056 &16.3858	&	0.3&	0.9 \\
16.5664 &20.4420	& 	0.4& 	0.9 \\
20.5566 &	27.2760 &	0.5	& 0.9 \\
50.7872 &	93.0302	 & 0.8 &	0.9 \\




N=70000

\begin{table}[hbtp]
\begin{tabular}{cccc} 
\hline
mean job &	mean batch& $q$	&$\rho^*$\\ \hline
2.8641 &	3.0707&	0,3&	0,5 \\
3.3635 &3.7137	& 	0,4& 	0,5 \\
3.9842 & 4.5563	 &	0,5	& 0,5 \\
10.1701 &	13.6023	 & 0,8 &	0,5\\
\hline
7.1308 &	8.3970 &	0.3 &	0.8 \\
8.3121 &	10.406 & 	0.4& 	0.8 \\
9.9831 &	13.3529 &	0.5	& 0.8 \\
24.9948 &	41.9611	 & 0.8 &	0.8 \\
\hline
13.1535 &15.2586	&	0,3&	0,9 \\
15.6862 &19.3887	& 	0,4& 	0,9 \\
20.3515 &	26.9405 &	0,5	& 0,9 \\
62.8132 &	116.5948	 & 0,8 &	0,9 \\
\hline
\end{tabular}
\end{table}





